Channel Charting: Locating Users within the Radio Environment using Channel State Information

We propose channel charting (CC), a novel framework in which a multi-antenna network element learns a chart of the radio geometry in its surrounding area. The channel chart captures the local spatial geometry of the area so that points that are close in space will also be close in the channel chart and vice versa. CC works in a fully unsupervised manner, i.e., learning is only based on channel state information (CSI) that is passively collected at a single point in space, but from multiple transmit locations in the area over time. The method then extracts channel features that characterize large-scale fading properties of the wireless channel. Finally, the channel charts are generated with tools from dimensionality reduction, manifold learning, and deep neural networks. The network element performing CC may be, for example, a multi-antenna base-station in a cellular system and the charted area in the served cell. Logical relationships related to the position and movement of a transmitter, e.g., a user equipment (UE), in the cell can then be directly deduced from comparing measured radio channel characteristics to the channel chart. The unsupervised nature of CC enables a range of new applications in UE localization, network planning, user scheduling, multipoint connectivity, hand-over, cell search, user grouping, and other cognitive tasks that rely on CSI and UE movement relative to the base-station, without the need of information from global navigation satellite systems.

==> macros.tex <==
%% ==============================================================
%% IIS-MIMO LaTeX Macros 
%% ==============================================================
%%
%% To be done:
%%  # definition remaining Greek matrices 
%%  # VLSI specific macros missing (process etc.)
%%
%% Version history:
%%   25-jul-2008   studer   update vectors and matrices
%%   24-apr-2008   studer   initial SVN check-in
%%
%% ==============================================================

%% -- References 
\renewcommand{\eqref}[1]{(\ref{#1})}
%\renewcommand{\eqref}[1]{Eq.~\ref{#1}}
\newcommand{\secref}[1]{\mbox{Section~\ref{#1}}}
%\newcommand{\secref}[1]{\mbox{Sec.~\ref{#1}}}
\newcommand{\appref}[1]{\mbox{Appendix~\ref{#1}}}
%\newcommand{\appref}[1]{\mbox{App.~\ref{#1}}}
\newcommand{\chapref}[1]{\mbox{Chapter~\ref{#1}}}
%\newcommand{\chapref}[1]{\mbox{Chap.~\ref{#1}}}
\newcommand{\figref}[1]{\mbox{Figure~\ref{#1}}}
%\newcommand{\figref}[1]{\mbox{Fig.~\ref{#1}}}
\newcommand{\tblref}[1]{\mbox{Table~\ref{#1}}}
%\newcommand{\tblref}[1]{\mbox{Tbl.~\ref{#1}}}
\newcommand{\algref}[1]{\mbox{Algorithm~\ref{#1}}}
%\newcommand{\algref}[1]{\mbox{Alg.~\ref{#1}}}

% -- USEFULL COMMANDS
\newcommand{\indexbf}[1]{\index{#1|textbf}}

%% -- Probabilities and densities
\renewcommand{\Pr}[1]{\ensuremath{\mathrm{P}\!\left[#1\right]}}
\newcommand{\Pe}[1]{\ensuremath{\mathrm{P_e}\!\left(#1\right)}}
\newcommand{\pr}[1]{\ensuremath{\mathrm{p}\!\left(#1\right)}}
\newcommand{\prG}[1]{\ensuremath{\mathrm{p}_\mathrm{G}\!\left(#1\right)}}
\newcommand{\PDF}[1]{\ensuremath{\mathrm{p}\!\left(#1\right)}}
\newcommand{\Ex}[1]{\ensuremath{\mathbb{E}\!\left[#1\right]}}
\newcommand{\Var}[1]{\ensuremath{\mathrm{Var}\!\left[#1\right]}}
\newcommand{\Q}[1]{\ensuremath{Q\!\left(#1\right)}}
\renewcommand{\mid}{\ensuremath{\,|\,}}

%% -- Operators
\DeclareMathOperator*{\logdet}{log\;det}
\DeclareMathOperator*{\logtwodet}{log_2\;det}
\DeclareMathOperator*{\argmin}{arg\;min}
\DeclareMathOperator*{\argmax}{arg\;max}
\DeclareMathOperator*{\arc}{arc}
\DeclareMathOperator*{\define}{\triangleq} 
\DeclareMathOperator*{\map}{map}
\DeclareMathOperator*{\invmap}{map^{-1}}

\newcommand{\sign}[1]{\ensuremath{\mathrm{sign}\!\left(#1\right)}}
%\newcommand{\sign}[1]{\ensuremath{\mathrm{sign}\!(#1)}}


%% -- Various math commands
\newcommand{\slice}[1]{\ensuremath{\mathrm{Q}\!\left(#1\right)}}
\newcommand{\COrder}[1]{\ensuremath{\mathcal{O}(#1)}}
\newcommand{\vecnorm}[1]{\ensuremath{\lVert#1\rVert}}
\newcommand{\adj}[1]{\ensuremath{\mathrm{adj}\,#1}}
\newcommand{\card}[1]{\ensuremath{|#1|}}
\newcommand{\abs}[1]{\ensuremath{\left|#1\right|}}
\newcommand{\expect}[1]{\ensuremath{\mathcal{E}\{#1\}}}
\newcommand{\NP}{\ensuremath{\mathcal{NP}}}
\newcommand{\eigv}[1]{\ensuremath{\lambda(#1)}}
\newcommand{\eigvmin}[1]{\ensuremath{\lambda_{\mathrm{min}}(#1)}}
\newcommand{\eigvmax}[1]{\ensuremath{\lambda_{\mathrm{max}}(#1)}}
\newcommand{\Cdim}[2]{\ensuremath{\in\mathbb{C}^{#1\times#2}}}
\newcommand{\Rdim}[2]{\ensuremath{\in\mathbb{R}^{#1\times#2}}}
\newcommand{\with}{\ensuremath{\quad\mathrm{with}\quad}}
\newcommand{\diag}[1]{\ensuremath{\mathrm{diag}\!\left(#1\right)}}
\newcommand{\atan}{\ensuremath{\mathrm{atan}}}
\newcommand{\Real}{\ensuremath{\mathbb{R}}}
\newcommand{\Complex}{\ensuremath{\mathbb{C}}}
\newcommand{\constant}{\ensuremath{\mathrm{const.}}}
\newcommand{\floor}[1]{\ensuremath{\left\lfloor#1\right\rfloor}}
\newcommand{\ceil}[1]{\ensuremath{\left\lceil#1\right\rceil}}
\newcommand{\round}[1]{\ensuremath{\left\lceil#1\right\rfloor}}

\newcommand{\ltwo}{\ensuremath{\ell^{2}}}
\newcommand{\lone}{\ensuremath{\ell^{1}}}
\newcommand{\linfty}{\ensuremath{\ell^{\infty}}}
\newcommand{\linftytilde}{\ensuremath{\ell^{\tilde{\infty}}}}

%% -- real and complex 
\newcommand{\C}{\ensuremath{\mathbb{C}}}
\newcommand{\R}{\ensuremath{\mathbb{R}}}
\newcommand{\Z}{\ensuremath{\mathbb{Z}}}
\newcommand{\CZ}{\ensuremath{\mathbb{CZ}}}

%% -- Sets
\newcommand{\setA}{\ensuremath{\mathcal{A}}}
\newcommand{\setB}{\ensuremath{\mathcal{B}}}
\newcommand{\setC}{\ensuremath{\mathcal{C}}}
\newcommand{\setD}{\ensuremath{\mathcal{D}}}
\newcommand{\setE}{\ensuremath{\mathcal{E}}}
\newcommand{\setF}{\ensuremath{\mathcal{F}}}
\newcommand{\setG}{\ensuremath{\mathcal{G}}}
\newcommand{\setH}{\ensuremath{\mathcal{H}}}
\newcommand{\setI}{\ensuremath{\mathcal{I}}}
\newcommand{\setJ}{\ensuremath{\mathcal{J}}}
\newcommand{\setK}{\ensuremath{\mathcal{K}}}
\newcommand{\setL}{\ensuremath{\mathcal{L}}}
\newcommand{\setM}{\ensuremath{\mathcal{M}}}
\newcommand{\setN}{\ensuremath{\mathcal{N}}}
\newcommand{\setO}{\ensuremath{\mathcal{O}}}
\newcommand{\setObar}{\ensuremath{\bar{\mathcal{O}}}}
\newcommand{\setP}{\ensuremath{\mathcal{P}}}
\newcommand{\setQ}{\ensuremath{\mathcal{Q}}}
\newcommand{\setR}{\ensuremath{\mathcal{R}}}
\newcommand{\setS}{\ensuremath{\mathcal{S}}}
\newcommand{\setT}{\ensuremath{\mathcal{T}}}
\newcommand{\setU}{\ensuremath{\mathcal{U}}}
\newcommand{\setV}{\ensuremath{\mathcal{V}}}
\newcommand{\setW}{\ensuremath{\mathcal{W}}}
\newcommand{\setX}{\ensuremath{\mathcal{X}}}
\newcommand{\setY}{\ensuremath{\mathcal{Y}}}
\newcommand{\setZ}{\ensuremath{\mathcal{Z}}}

%% -- Bold lower-case letters: vectors
\newcommand{\bma}{\ensuremath{\mathbf{a}}}
\newcommand{\bmb}{\ensuremath{\mathbf{b}}}
\newcommand{\bmc}{\ensuremath{\mathbf{c}}}
\newcommand{\bmd}{\ensuremath{\mathbf{d}}}
\newcommand{\bme}{\ensuremath{\mathbf{e}}}
\newcommand{\bmf}{\ensuremath{\mathbf{f}}}
\newcommand{\bmg}{\ensuremath{\mathbf{g}}}
\newcommand{\bmh}{\ensuremath{\mathbf{h}}}
\newcommand{\bmi}{\ensuremath{\mathbf{i}}}
\newcommand{\bmj}{\ensuremath{\mathbf{j}}}
\newcommand{\bmk}{\ensuremath{\mathbf{k}}}
\newcommand{\bml}{\ensuremath{\mathbf{l}}}
\newcommand{\bmm}{\ensuremath{\mathbf{m}}}
\newcommand{\bmn}{\ensuremath{\mathbf{n}}}
\newcommand{\bmo}{\ensuremath{\mathbf{o}}}
\newcommand{\bmp}{\ensuremath{\mathbf{p}}}
\newcommand{\bmq}{\ensuremath{\mathbf{q}}}
\newcommand{\bmr}{\ensuremath{\mathbf{r}}}
\newcommand{\bms}{\ensuremath{\mathbf{s}}}
\newcommand{\bmt}{\ensuremath{\mathbf{t}}}
\newcommand{\bmu}{\ensuremath{\mathbf{u}}}
\newcommand{\bmv}{\ensuremath{\mathbf{v}}}
\newcommand{\bmw}{\ensuremath{\mathbf{w}}}
\newcommand{\bmx}{\ensuremath{\mathbf{x}}}
\newcommand{\bmy}{\ensuremath{\mathbf{y}}}
\newcommand{\bmz}{\ensuremath{\mathbf{z}}}
\newcommand{\bmone}{\ensuremath{\mathbf{1}}}
\newcommand{\bmzero}{\ensuremath{\mathbf{0}}}

%% -- vectors with hat
\newcommand{\bmahat}{\ensuremath{\hat{\bma}}}
\newcommand{\bmbhat}{\ensuremath{\hat{\bmb}}}
\newcommand{\bmchat}{\ensuremath{\hat{\bmc}}}
\newcommand{\bmdhat}{\ensuremath{\hat{\bmd}}}
\newcommand{\bmehat}{\ensuremath{\hat{\bme}}}
\newcommand{\bmfhat}{\ensuremath{\hat{\bmf}}}
\newcommand{\bmghat}{\ensuremath{\hat{\bmg}}}
\newcommand{\bmhhat}{\ensuremath{\hat{\bmh}}}
\newcommand{\bmihat}{\ensuremath{\hat{\bmi}}}
\newcommand{\bmjhat}{\ensuremath{\hat{\bmj}}}
\newcommand{\bmkhat}{\ensuremath{\hat{\bmk}}}
\newcommand{\bmlhat}{\ensuremath{\hat{\bml}}}
\newcommand{\bmmhat}{\ensuremath{\hat{\bmm}}}
\newcommand{\bmnhat}{\ensuremath{\hat{\bmn}}}
\newcommand{\bmohat}{\ensuremath{\hat{\bmo}}}
\newcommand{\bmphat}{\ensuremath{\hat{\bmp}}}
\newcommand{\bmqhat}{\ensuremath{\hat{\bmq}}}
\newcommand{\bmrhat}{\ensuremath{\hat{\bmr}}}
\newcommand{\bmshat}{\ensuremath{\hat{\bms}}}
\newcommand{\bmthat}{\ensuremath{\hat{\bmt}}}
\newcommand{\bmuhat}{\ensuremath{\hat{\bmu}}}
\newcommand{\bmvhat}{\ensuremath{\hat{\bmv}}}
\newcommand{\bmwhat}{\ensuremath{\hat{\bmw}}}
\newcommand{\bmxhat}{\ensuremath{\hat{\bmx}}}
\newcommand{\bmyhat}{\ensuremath{\hat{\bmy}}}
\newcommand{\bmzhat}{\ensuremath{\hat{\bmz}}}

%% -- Vectors with tilde
\newcommand{\bmatilde}{\ensuremath{\tilde{\bma}}}
\newcommand{\bmbtilde}{\ensuremath{\tilde{\bmb}}}
\newcommand{\bmctilde}{\ensuremath{\tilde{\bmc}}}
\newcommand{\bmdtilde}{\ensuremath{\tilde{\bmd}}}
\newcommand{\bmetilde}{\ensuremath{\tilde{\bme}}}
\newcommand{\bmftilde}{\ensuremath{\tilde{\bmf}}}
\newcommand{\bmgtilde}{\ensuremath{\tilde{\bmg}}}
\newcommand{\bmhtilde}{\ensuremath{\tilde{\bmh}}}
\newcommand{\bmitilde}{\ensuremath{\tilde{\bmi}}}
\newcommand{\bmjtilde}{\ensuremath{\tilde{\bmj}}}
\newcommand{\bmktilde}{\ensuremath{\tilde{\bmk}}}
\newcommand{\bmltilde}{\ensuremath{\tilde{\bml}}}
\newcommand{\bmmtilde}{\ensuremath{\tilde{\bmm}}}
\newcommand{\bmntilde}{\ensuremath{\tilde{\bmn}}}
\newcommand{\bmotilde}{\ensuremath{\tilde{\bmo}}}
\newcommand{\bmptilde}{\ensuremath{\tilde{\bmp}}}
\newcommand{\bmqtilde}{\ensuremath{\tilde{\bmq}}}
\newcommand{\bmrtilde}{\ensuremath{\tilde{\bmr}}}
\newcommand{\bmstilde}{\ensuremath{\tilde{\bms}}}
\newcommand{\bmttilde}{\ensuremath{\tilde{\bmt}}}
\newcommand{\bmutilde}{\ensuremath{\tilde{\bmu}}}
\newcommand{\bmvtilde}{\ensuremath{\tilde{\bmv}}}
\newcommand{\bmwtilde}{\ensuremath{\tilde{\bmw}}}
\newcommand{\bmxtilde}{\ensuremath{\tilde{\bmx}}}
\newcommand{\bmytilde}{\ensuremath{\tilde{\bmy}}}
\newcommand{\bmztilde}{\ensuremath{\tilde{\bmz}}}

%% -- Vectors with bar
\newcommand{\bmabar}{\ensuremath{\bar{\bma}}}
\newcommand{\bmbbar}{\ensuremath{\bar{\bmb}}}
\newcommand{\bmcbar}{\ensuremath{\bar{\bmc}}}
\newcommand{\bmdbar}{\ensuremath{\bar{\bmd}}}
\newcommand{\bmebar}{\ensuremath{\bar{\bme}}}
\newcommand{\bmfbar}{\ensuremath{\bar{\bmf}}}
\newcommand{\bmgbar}{\ensuremath{\bar{\bmg}}}
\newcommand{\bmhbar}{\ensuremath{\bar{\bmh}}}
\newcommand{\bmibar}{\ensuremath{\bar{\bmi}}}
\newcommand{\bmjbar}{\ensuremath{\bar{\bmj}}}
\newcommand{\bmkbar}{\ensuremath{\bar{\bmk}}}
\newcommand{\bmlbar}{\ensuremath{\bar{\bml}}}
\newcommand{\bmmbar}{\ensuremath{\bar{\bmm}}}
\newcommand{\bmnbar}{\ensuremath{\bar{\bmn}}}
\newcommand{\bmobar}{\ensuremath{\bar{\bmo}}}
\newcommand{\bmpbar}{\ensuremath{\bar{\bmp}}}
\newcommand{\bmqbar}{\ensuremath{\bar{\bmq}}}
\newcommand{\bmrbar}{\ensuremath{\bar{\bmr}}}
\newcommand{\bmsbar}{\ensuremath{\bar{\bms}}}
\newcommand{\bmtbar}{\ensuremath{\bar{\bmt}}}
\newcommand{\bmubar}{\ensuremath{\bar{\bmu}}}
\newcommand{\bmvbar}{\ensuremath{\bar{\bmv}}}
\newcommand{\bmwbar}{\ensuremath{\bar{\bmw}}}
\newcommand{\bmxbar}{\ensuremath{\bar{\bmx}}}
\newcommand{\bmybar}{\ensuremath{\bar{\bmy}}}
\newcommand{\bmzbar}{\ensuremath{\bar{\bmz}}}

%% -- Bold upper-case letters: matrices
\newcommand{\bA}{\ensuremath{\mathbf{A}}}
\newcommand{\bB}{\ensuremath{\mathbf{B}}}
\newcommand{\bC}{\ensuremath{\mathbf{C}}}
\newcommand{\bD}{\ensuremath{\mathbf{D}}}
\newcommand{\bE}{\ensuremath{\mathbf{E}}}
\newcommand{\bF}{\ensuremath{\mathbf{F}}}
\newcommand{\bG}{\ensuremath{\mathbf{G}}}
\newcommand{\bH}{\ensuremath{\mathbf{H}}}
\newcommand{\bI}{\ensuremath{\mathbf{I}}}
\newcommand{\bJ}{\ensuremath{\mathbf{J}}}
\newcommand{\bK}{\ensuremath{\mathbf{K}}}
\newcommand{\bL}{\ensuremath{\mathbf{L}}}
\newcommand{\bM}{\ensuremath{\mathbf{M}}}
\newcommand{\bN}{\ensuremath{\mathbf{N}}}
\newcommand{\bO}{\ensuremath{\mathbf{O}}}
\newcommand{\bP}{\ensuremath{\mathbf{P}}}
\newcommand{\bQ}{\ensuremath{\mathbf{Q}}}
\newcommand{\bR}{\ensuremath{\mathbf{R}}}
\newcommand{\bS}{\ensuremath{\mathbf{S}}}
\newcommand{\bT}{\ensuremath{\mathbf{T}}}
\newcommand{\bU}{\ensuremath{\mathbf{U}}}
\newcommand{\bV}{\ensuremath{\mathbf{V}}}
\newcommand{\bW}{\ensuremath{\mathbf{W}}}
\newcommand{\bX}{\ensuremath{\mathbf{X}}}
\newcommand{\bY}{\ensuremath{\mathbf{Y}}}
\newcommand{\bZ}{\ensuremath{\mathbf{Z}}}
\newcommand{\bZero}{\ensuremath{\mathbf{0}}}
\newcommand{\bOne}{\ensuremath{\mathbf{1}}}
\newcommand{\bPsi}{\ensuremath{\mathbf{\Psi}}}
\newcommand{\bGamma}{\ensuremath{\mathbf{\Gamma}}}
\newcommand{\bTheta}{\ensuremath{\mathbf{\Theta}}}
\newcommand{\bLambda}{\ensuremath{\mathbf{\Lambda}}}
\newcommand{\bDelta}{\ensuremath{\mathbf{\Delta}}}
\newcommand{\bSigma}{\ensuremath{\mathbf{\Sigma}}}
\newcommand{\bBeta}{\ensuremath{\underline{\beta}}}

%% -- Bold upper-case letters: matrices with hat
\newcommand{\bAhat}{\ensuremath{\hat{\mathbf{A}}}}
\newcommand{\bBhat}{\ensuremath{\hat{\mathbf{B}}}}
\newcommand{\bChat}{\ensuremath{\hat{\mathbf{C}}}}
\newcommand{\bDhat}{\ensuremath{\hat{\mathbf{D}}}}
\newcommand{\bEhat}{\ensuremath{\hat{\mathbf{E}}}}
\newcommand{\bFhat}{\ensuremath{\hat{\mathbf{F}}}}
\newcommand{\bGhat}{\ensuremath{\hat{\mathbf{G}}}}
\newcommand{\bHhat}{\ensuremath{\hat{\mathbf{H}}}}
\newcommand{\bIhat}{\ensuremath{\hat{\mathbf{I}}}}
\newcommand{\bJhat}{\ensuremath{\hat{\mathbf{J}}}}
\newcommand{\bKhat}{\ensuremath{\hat{\mathbf{K}}}}
\newcommand{\bLhat}{\ensuremath{\hat{\mathbf{L}}}}
\newcommand{\bMhat}{\ensuremath{\hat{\mathbf{M}}}}
\newcommand{\bNhat}{\ensuremath{\hat{\mathbf{N}}}}
\newcommand{\bOhat}{\ensuremath{\hat{\mathbf{O}}}}
\newcommand{\bPhat}{\ensuremath{\hat{\mathbf{P}}}}
\newcommand{\bQhat}{\ensuremath{\hat{\mathbf{Q}}}}
\newcommand{\bRhat}{\ensuremath{\hat{\mathbf{R}}}}
\newcommand{\bShat}{\ensuremath{\hat{\mathbf{S}}}}
\newcommand{\bThat}{\ensuremath{\hat{\mathbf{T}}}}
\newcommand{\bUhat}{\ensuremath{\hat{\mathbf{U}}}}
\newcommand{\bVhat}{\ensuremath{\hat{\mathbf{V}}}}
\newcommand{\bWhat}{\ensuremath{\hat{\mathbf{W}}}}
\newcommand{\bXhat}{\ensuremath{\hat{\mathbf{X}}}}
\newcommand{\bYhat}{\ensuremath{\hat{\mathbf{Y}}}}
\newcommand{\bZhat}{\ensuremath{\hat{\mathbf{Z}}}}
\newcommand{\bZerohat}{\ensuremath{\hat{\mathbf{0}}}}
\newcommand{\bOnehat}{\ensuremath{\hat{\mathbf{1}}}}
\newcommand{\bPsihat}{\ensuremath{\hat{\mathbf{\Psi}}}}
\newcommand{\bThetahat}{\ensuremath{\hat{\mathbf{\Theta}}}}
\newcommand{\bLambdahat}{\ensuremath{\hat{\mathbf{\Lambda}}}}
\newcommand{\bDeltahat}{\ensuremath{\hat{\mathbf{\Delta}}}}
\newcommand{\bSigmahat}{\ensuremath{\hat{\mathbf{\Sigma}}}}

%% -- Bold upper-case letters: matrices with tilde
\newcommand{\bAtilde}{\ensuremath{\widetilde{\mathbf{A}}}}
\newcommand{\bBtilde}{\ensuremath{\widetilde{\mathbf{B}}}}
\newcommand{\bCtilde}{\ensuremath{\widetilde{\mathbf{C}}}}
\newcommand{\bDtilde}{\ensuremath{\widetilde{\mathbf{D}}}}
\newcommand{\bEtilde}{\ensuremath{\widetilde{\mathbf{E}}}}
\newcommand{\bFtilde}{\ensuremath{\widetilde{\mathbf{F}}}}
\newcommand{\bGtilde}{\ensuremath{\widetilde{\mathbf{G}}}}
\newcommand{\bHtilde}{\ensuremath{\widetilde{\mathbf{H}}}}
\newcommand{\bItilde}{\ensuremath{\widetilde{\mathbf{I}}}}
\newcommand{\bJtilde}{\ensuremath{\widetilde{\mathbf{J}}}}
\newcommand{\bKtilde}{\ensuremath{\widetilde{\mathbf{K}}}}
\newcommand{\bLtilde}{\ensuremath{\widetilde{\mathbf{L}}}}
\newcommand{\bMtilde}{\ensuremath{\widetilde{\mathbf{M}}}}
\newcommand{\bNtilde}{\ensuremath{\widetilde{\mathbf{N}}}}
\newcommand{\bOtilde}{\ensuremath{\widetilde{\mathbf{O}}}}
\newcommand{\bPtilde}{\ensuremath{\widetilde{\mathbf{P}}}}
\newcommand{\bQtilde}{\ensuremath{\widetilde{\mathbf{Q}}}}
\newcommand{\bRtilde}{\ensuremath{\widetilde{\mathbf{R}}}}
\newcommand{\bStilde}{\ensuremath{\widetilde{\mathbf{S}}}}
\newcommand{\bTtilde}{\ensuremath{\widetilde{\mathbf{T}}}}
\newcommand{\bUtilde}{\ensuremath{\widetilde{\mathbf{U}}}}
\newcommand{\bVtilde}{\ensuremath{\widetilde{\mathbf{V}}}}
\newcommand{\bWtilde}{\ensuremath{\widetilde{\mathbf{W}}}}
\newcommand{\bXtilde}{\ensuremath{\widetilde{\mathbf{X}}}}
\newcommand{\bYtilde}{\ensuremath{\widetilde{\mathbf{Y}}}}
\newcommand{\bZtilde}{\ensuremath{\widetilde{\mathbf{Z}}}}
\newcommand{\bZerotilde}{\ensuremath{\widetilde{\mathbf{0}}}}
\newcommand{\bOnetilde}{\ensuremath{\widetilde{\mathbf{1}}}}
\newcommand{\bPsitilde}{\ensuremath{\widetilde{\mathbf{\Psi}}}}
\newcommand{\bThetatilde}{\ensuremath{\widetilde{\mathbf{\Theta}}}}
\newcommand{\bLambdatilde}{\ensuremath{\widetilde{\mathbf{\Lambda}}}}
\newcommand{\bDeltatilde}{\ensuremath{\widetilde{\mathbf{\Delta}}}}
\newcommand{\bSigmatilde}{\ensuremath{\widetilde{\mathbf{\Sigma}}}}

%% -- Bold upper-case letters: matrices with bar
\newcommand{\bAbar}{\ensuremath{\bar{\mathbf{A}}}}
\newcommand{\bBbar}{\ensuremath{\bar{\mathbf{B}}}}
\newcommand{\bCbar}{\ensuremath{\bar{\mathbf{C}}}}
\newcommand{\bDbar}{\ensuremath{\bar{\mathbf{D}}}}
\newcommand{\bEbar}{\ensuremath{\bar{\mathbf{E}}}}
\newcommand{\bFbar}{\ensuremath{\bar{\mathbf{F}}}}
\newcommand{\bGbar}{\ensuremath{\bar{\mathbf{G}}}}
\newcommand{\bHbar}{\ensuremath{\bar{\mathbf{H}}}}
\newcommand{\bIbar}{\ensuremath{\bar{\mathbf{I}}}}
\newcommand{\bJbar}{\ensuremath{\bar{\mathbf{J}}}}
\newcommand{\bKbar}{\ensuremath{\bar{\mathbf{K}}}}
\newcommand{\bLbar}{\ensuremath{\bar{\mathbf{L}}}}
\newcommand{\bMbar}{\ensuremath{\bar{\mathbf{M}}}}
\newcommand{\bNbar}{\ensuremath{\bar{\mathbf{N}}}}
\newcommand{\bObar}{\ensuremath{\bar{\mathbf{O}}}}
\newcommand{\bPbar}{\ensuremath{\bar{\mathbf{P}}}}
\newcommand{\bQbar}{\ensuremath{\bar{\mathbf{Q}}}}
\newcommand{\bRbar}{\ensuremath{\bar{\mathbf{R}}}}
\newcommand{\bSbar}{\ensuremath{\bar{\mathbf{S}}}}
\newcommand{\bTbar}{\ensuremath{\bar{\mathbf{T}}}}
\newcommand{\bUbar}{\ensuremath{\bar{\mathbf{U}}}}
\newcommand{\bVbar}{\ensuremath{\bar{\mathbf{V}}}}
\newcommand{\bWbar}{\ensuremath{\bar{\mathbf{W}}}}
\newcommand{\bXbar}{\ensuremath{\bar{\mathbf{X}}}}
\newcommand{\bYbar}{\ensuremath{\bar{\mathbf{Y}}}}
\newcommand{\bZbar}{\ensuremath{\bar{\mathbf{Z}}}}
\newcommand{\bZerobar}{\ensuremath{\bar{\mathbf{0}}}}
\newcommand{\bOnebar}{\ensuremath{\bar{\mathbf{1}}}}
\newcommand{\bPsibar}{\ensuremath{\bar{\mathbf{\Psi}}}}
\newcommand{\bThetabar}{\ensuremath{\bar{\mathbf{\Theta}}}}
\newcommand{\bDeltabar}{\ensuremath{\bar{\mathbf{\Delta}}}}
\newcommand{\bSigmabar}{\ensuremath{\bar{\mathbf{\Sigma}}}}

%% -- MIMO and coding specific macros
\newcommand{\MT}{{\ensuremath{U}}}
\newcommand{\MR}{{\ensuremath{B}}}
\newcommand{\SNR}{\ensuremath{\mathsf{SNR}}}
\newcommand{\SQNR}{\ensuremath{\mathsf{SQNR}}}
\newcommand{\SINR}{\ensuremath{\mathsf{SINR}}}
\newcommand{\const}{\ensuremath{\setO}}
\newcommand{\modorder}{\ensuremath{Q}}
\newcommand{\Pn}{\ensuremath{\sigma^{2}}}
\newcommand{\No}{\ensuremath{N_{\mathrm{0}}}}
\newcommand{\dmin}{{\ensuremath{d_\mathrm{min}}}}
\newcommand{\Es}{{\ensuremath{E_{\mathrm{s}}}}}
\newcommand{\Eb}{{\ensuremath{E_{\mathrm{b}}}}}

% -- LLRs
\newcommand{\LA}{L^\mathrm{A}}
\newcommand{\LD}{L^\mathrm{D}}
\newcommand{\LE}{L^\mathrm{E}}
\newcommand{\LC}{L^\mathrm{C}}
\newcommand{\LAtilde}{\tilde{L}^\mathrm{A}}
\newcommand{\LDtilde}{\tilde{L}^\mathrm{D}}
\newcommand{\LEtilde}{\tilde{L}^\mathrm{E}}
\newcommand{\LAbar}{\bar{L}^\mathrm{A}}
\newcommand{\LDbar}{\bar{L}^\mathrm{D}}
\newcommand{\LEbar}{\bar{L}^\mathrm{E}}
\newcommand{\LAm}{L^{\mathrm{A1}}}
\newcommand{\LDm}{L^{\mathrm{D1}}}
\newcommand{\LEm}{L^{\mathrm{E1}}}
\newcommand{\LAEm}{L^{\mathrm{AE1}}}
\newcommand{\LADm}{L^{\mathrm{AD1}}}
\newcommand{\LAc}{L^{\mathrm{A2}}}
\newcommand{\LDc}{L^{\mathrm{D2}}}
\newcommand{\LEc}{L^{\mathrm{E2}}}
\newcommand{\NIT}{I}

% -- detection specific
\newcommand{\ML}{{\ensuremath{\mathrm{ML}}}}
\newcommand{\MLbar}{{\ensuremath{\overline{\mathrm{ML}}}}}
\newcommand{\MAP}{{\ensuremath{\mathrm{MAP}}}}
\newcommand{\MAPbar}{{\ensuremath{\overline{\mathrm{MAP}}}}}
\newcommand{\SIC}{{\ensuremath{\mathrm{SIC}}}}
\newcommand{\ZF}{{\ensuremath{\mathrm{ZF}}}}
\newcommand{\MMSE}{{\ensuremath{\mathrm{MMSE}}}}
\newcommand{\MF}{{\ensuremath{\mathrm{MF}}}}

%% -- VLSI specific macos
\newcommand{\tclk}{\ensuremath{t_\mathrm{clk}}}
\newcommand{\fclk}{\ensuremath{f_\mathrm{clk}}}
\newcommand{\AT}{\ensuremath{\mathit{AT}}}
\newcommand{\ATPP}{\ensuremath{\mathit{AT}_\mathrm{pp}}}
\newcommand{\ATM}{\ensuremath{\mathit{AT}_\mathrm{m}}}
\newcommand{\ATC}{\ensuremath{\mathit{AT}_\mathrm{c}}}
\newcommand{\ATS}{\ensuremath{\mathit{AT}_\mathrm{s}}}
\newcommand{\Area}{\ensuremath{\mathit{A}}}
\newcommand{\AreaPP}{\ensuremath{\mathit{A}_\mathrm{pp}}}
\newcommand{\AreaM}{\ensuremath{\mathit{A}_\mathrm{m}}}
\newcommand{\AreaC}{\ensuremath{\mathit{A}_\mathrm{c}}}
\newcommand{\TP}{\ensuremath{\Theta}}
\newcommand{\TPM}{\ensuremath{\Theta_\mathrm{m}}}
\newcommand{\TPC}{\ensuremath{\Theta_\mathrm{c}}}

%% -- Complexities macros
\newcommand{\CGr}{\ensuremath{C_{\mathrm{GR}}}}
\newcommand{\CVec}{\ensuremath{C_{\mathrm{Vec}}}}
\newcommand{\CRot}{\ensuremath{C_{\mathrm{Rot}}}}
\newcommand{\CMult}{\ensuremath{C_{\mathrm{Mult}}}}
\newcommand{\COMult}{\ensuremath{C_{\mathrm{OptMult}}}}
\newcommand{\CDiv}{\ensuremath{C_{\mathrm{Div}}}}
\newcommand{\CSqrt}{\ensuremath{C_{\sqrt{\cdot}}}}

% -- lattice reduction macros

\newcommand{\DREL}{{\ensuremath{\underline{D}}}}
\newcommand{\CREL}{{\ensuremath{\underline{C}}}}
\newcommand{\rREL}{{\ensuremath{\underline{r}}}}
\newcommand{\LR}{{\ensuremath{\mathrm{LR}}}}
\newcommand{\bmxREL}{{\ensuremath{\underline{\mathbf{x}}}}} 
\newcommand{\bmuREL}{{\ensuremath{\underline{\mathbf{u}}}}}
\newcommand{\bmuhatREL}{{\ensuremath{\hat{\underline{\mathbf{u}}}}}} 
\newcommand{\bmxhatREL}{{\ensuremath{\hat{\underline{\mathbf{x}}}}}} 
\newcommand{\CZMT}{{\ensuremath{(\CZ)^{\MT}}}} 
\newcommand{\LatticeREL}{{\ensuremath{\underline{\setL}}}} 
\newcommand{\Lattice}{{\ensuremath{\setL}}}
\newcommand{\BABAI}{{\ensuremath{\mathrm{B}}}}

% -- STS specific
\newcommand{\IEmap}[1]{f\!\left(#1\right)} % map from intrinsic to extrinsic
\newcommand{\EImap}[1]{f^{-1}\!\left(#1\right)} % map from extrinsic to intrinsic
\newcommand{\fc}{{g}}
\newcommand{\fctilde}{{\tilde{g}}}
\newcommand{\IA}{{I_\mathrm{A}}}
\newcommand{\IE}{{I_\mathrm{E}}}
\newcommand{\Lmax}{{L_\mathrm{max}}}

% -- MISC
\newtheorem{thm}{Theorem}
\newtheorem{lem}[thm]{Lemma}
\makeatletter
\renewenvironment{proof}[1][\proofname]{\par
  \pushQED{\qed}%
  \normalfont \topsep6\p@\@plus6\p@\relax
  \trivlist
  %\itemindent\normalparindent
  \item[\hskip\labelsep
        \scshape
    #1\@addpunct{.}]\ignorespaces
}{%
  \popQED\endtrivlist\@endpefalse
}
\makeatother


